StylePeople: A Generative Model of Fullbody Human Avatars

We propose a new type of full-body human avatars, which combines parametric mesh-based body model with a neural texture. We show that with the help of neural textures, such avatars can successfully model clothing and hair, which usually poses a problem for mesh-based approaches. We also show how these avatars can be created from multiple frames of a video using backpropagation. We then propose a generative model for such avatars that can be trained from datasets of images and videos of people. The generative model allows us to sample random avatars as well as to create dressed avatars of people from one or few images. The code for the project is available at saic-violet.github.io/style-people.

==> impact.tex <==
\section*{Broader Impact}

Realistic modeling of human appearance has multiple benign implications. Perhaps the most important one is the increased realism of virtual reality and augmented reality telepresence systems. As of now, non-photorealistic avatars are used in such systems. Other applications include gaming and, eventually, with the increased level of realism, special effects in cinematography. Of course, as soon as the realism becomes very high, the mass-spread of ``full body'' deep fake videos may become a problem. Watermarking and advanced fake detection techniques should be developed to counter this threat. What is the best way to incorporate watermarking into our approach, is an interesting research question, and the respective modification of the rendering network seems the most obvious solution.
